Fast-ELECTRA for Efficient Pre-training

ELECTRA pre-trains language models by detecting tokens in a sequence that have been replaced by an auxiliary model. Although ELECTRA offers a significant boost in efficiency, its potential is constrained by the training cost brought by the auxiliary model. Notably, this model, which is jointly trained with the main model, only serves to assist the training of the main model and is discarded post-training. This results in a substantial amount of training cost being expended in vain. To mitigate this issue, we propose Fast-ELECTRA, which leverages an existing language model as the auxiliary model. To construct a learning curriculum for the main model, we smooth its output distribution via temperature scaling following a descending schedule. Our approach rivals the performance of state-of-the-art ELECTRA-style pre-training methods, while significantly eliminating the computation and memory cost brought by the joint training of the auxiliary model. Our method also reduces the sensitivity to hyper-parameters and enhances the pre-training stability.

==> backups/robustness-backup.tex <==
% \subsection{Robustness to the Learning Curriculum}
\subsection{Robustness to the Hyper-parameter Settings}
\label{sect:robustness}


% \todo{Dont have to mention curriculum here}
% \todo{Have to mention learning curriculum here as we didn't mention it in the method section}
% \todo{Abstract the detail of trajectory here, then actually don't have to elaborate the details in the method section.}

In this section, we investigate the robustness of our method to the hyper-parameter settings. We are mostly interested in the hyper-parameters controlling the learning curriculum in the RTD task, since it is the key difference between \ours{} and the original ELECTRA and is also important to the effectiveness of ELECTRA-style pre-training.

In ELECTRA, the learning curriculum is characterized by the difficulty of the replaced token detection task throughout the pre-training, which we refer to as the difficulty trajectory. Controlling the learning curriculum is challenging because a difficulty trajectory that is positive in the short term is not necessarily beneficial in the long term. Searching for the optimal difficulty trajectory often requires pre-training till the end.
Controlling the learning curriculum is particularly challenging for pre-training because the effectiveness of a difficulty trajectory can only be revealed by the performance on representative downstream tasks, which requires time-consuming fine-tuning. There is no reliable signal through pre-training that can instantly indicate the effect of a difficulty trajectory.
% Therefore, in practice we would strongly prefer a curriculum control that is robust to the hyper-parameter setting.
Therefore, in practice, we would strongly prefer an ELECTRA-style pre-training method that is more friendly for tuning the learning curriculum.


\input{figures/robustness}


\todo{Friendly: Unimodal and insensitive}



% \smallsection{Difficulty Trajectory controlled by the Generator Capacity}
\smallsection{Generator Capacity}
The generator capacity can also implicitly control the difficulty trajectory. A large generator can converge faster~\citep{Arora2018ACA}, thus creating a more difficult task for the discriminator. Previous works have observed that a generator that is too large or too small can both damage the effectiveness of the pre-training~\citep{Clark2020ELECTRAPT}.
% Optimal pre-training performance requires a generator that is neither too strong nor too weak.
However, tuning the generator capacity in practice can induce significantly more effort than tuning other hyper-parameters, as the model architecture changes in each training trial, which means the experiment or hardware setup very likely needs to be re-configured to debug training and maintain efficiency. 

We show that \ours{} can reduce the sensitivity of the pre-training effectiveness to the generator capacity, thus being more friendly to use in practice. We experiment on the original ELECTRA and \ours{} with varying generator depths, while for other difficulty controlling hyper-parameters (\emph{i.e.,} loss weight in the original ELECTRA and decay rate in \ours{}) we select the ones that produce the best performance for each depth respectively.
As shown in Figure~\ref{figure:robustness-gen-depth}, \ours{} can reduce the performance gap between a carefully selected generator ($4$-layer) and a generator doubling the size ($8$-layer).
% \note{\ours{} can achieve similar performance when doubling the number of layers compared to a carefully selected generator size ($4$ layers)}. 
% \ours{} can also alleviate the performance reduction when using a generator that is as large as the discriminator. In contrast, the performance of the original ELECTRA design quickly decreases as the generator capacity increases.
In addition, \ours{} can also achieve better downstream performance consistently for all generator sizes.

\todo{Add 6-layer main model?}


% As mentioned in Section~\ref{sect:method}, the learning curriculum in ELECTRA-style pre-training is entirely defined by the trajectory of the replaced token distribution, namely $p_G(t; w|c)$.







\smallsection{Explicit Modulation of the Difficulty Trajectory}

\todo{Original: Loss weight: 30, 40, \textbf{50}, 60, \textbf{70}, 80}
% CE + $\lambda$ BCE, with a loss scale trick, with $5$ as a step size
\todo{\ours{}: $\tau$: \textbf{0.05}, \textbf{0.1}, 0.3, \textbf{0.5}, 0.7}


\todo{show two sets of generator size, to see tuning from 50 to 70 is necessary. Ideally, we should show the large here, but probably don't have the results.}
\todo{The change is both smooth and uni-modal, which is also important for friendly hyper-parameter tuning}

\chengyu{we choose these hyper-parameters for baseline because they are the necessary grid search range for different training setups (e.g., different generator sizes). We choose these hyperparameters }


% Now two hyper-parameters, previous more hyper-parameters.
% Fast-ELECTRA is also more friendly for hyper-parameter search as the learning curriculum is now completely determined by two hyper-parameters, while previously it depends on multiple hyper-parameters such as the loss weight and those for optimizing the auxiliary model including learning rate, warm up, etc.
% Based on extensive experiments, 
We show that \ours{} is more robust to the variation of the difficulty trajectory, thus can significantly reduce the trial-and-error effort in practice.
Following previous works~\citep{Bajaj2022METROED}, we measure the difficulty of the replaced token detection task by \emph{replace rate}, namely the fraction of replaced tokens among all the input tokens fed to the main model. For the convenience of analysis, we further characterize the difficulty trajectory by the average replace rate over all checkpoints~\footnote{Note that this essentially defines a functional that maps a trajectory function to a single number.}, which reflects the overall difficulty of the replaced token detection task through pre-training. 
% Note that this is not necessarily a genunie measure of the difficulty considering the semantics.
% a generator’s MLM predictions on the 15\% masked positions.

In Figure~\ref{figure:robustness-replace-rate}, we experiment on the original ELECTRA with a varying difficulty schedule, which is modulated by the loss weight designed to balance the optimizations of the discriminator (main model) and the generator (auxiliary model).
% and the learning rate $\eta$. % Note that the learning rate is tricky as it will also affect the discriminator learning.
 One can find that the downstream performance changes abruptly when the difficulty trajectory varies. 
 % , characterized by 
 % both the replace rate at the last checkpoint and 
 % the average replace rate over all checkpoints. 
 In contrast, \ours{} significantly reduce the sensitivity of the downstream performance to the variation of the difficulty schedule (modulated by the decay rate of the temperature as mentioned in Section~\ref{sect:method}).
% , which introduces two hyper-parameters, including the initial temperature and the decay rate. 






% \todo{Figure}
% \begin{itemize}
%     \item Performance vs. generator sizes over a fixed hyperparameter setting
%     \item Performance vs. generator sizes over the best hyperparameter setting for each generator
% \end{itemize}

% \sout{No need to balance loss (loss weight is critical in previous setting) But how to showcase this?}
% More tolerant to discriminator training hyperparameters?
% \begin{itemize}
%     \item Learning rate and other optimization hyperparameters
% \end{itemize}

% Much fewer generator hyperparameters need to be tuned compared to previous training method:
% \begin{itemize}
%     \item Original ELECTRA: loss weight, generator training hyperparameters (learning rate, warm up, etc.)
%     % \item Decoupled ELECTRA (generator training hyperparameters)
%     \item Our method: Initial weight and decay rate in the schedule function. No hyperparameter in the augmentation function.
% \end{itemize}

% Tips for selecting hyper-parameters:
% \begin{itemize}
%     \item Initial weight can be largely determined based on the initial nll loss (between 10-14) or replace rate (0.15).
%     % \item The final performance is also not sensitive to the initial weight given current experiments on dropout-w-attention. \#ToCheck
%     \item Initial temperature = 2 is the best for almost all settings.
%     \item So the only hyper-parameter needs to be tuned is the decay rate.
% \end{itemize}

==> figures/stability.tex <==
% \begin{figure}[htbp]
\begin{wrapfigure}{R}{0.5\textwidth} % R instead of r to avoid overflow
\vspace{-6mm}
     \centering
     \includegraphics[width=1.0\linewidth]{figures/stability-lr.pdf}
    \caption{
         Training loss curves of the main model when pre-training with the original ELECTRA (\emph{Left}) and \ours{} (\emph{Right}).
         % for BERT-base equivalent models pre-trained with the ``Original'' ELECTRA design and our ``\ours{}''. 
        ``$\times$'' indicates the divergence of the training.
    }
    \label{figure:stability-lr}
% \end{figure}
\vspace{-3mm}
\end{wrapfigure}

==> inputs/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{See Section~\ref{sect:limitation}}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerYes{See Section~\ref{sect:limitation}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{}
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    % \answerTODO{}
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    % \answerTODO{}
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerTODO{}
    \answerYes{}
  \item Did you mention the license of the assets?
    % \answerTODO{}
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    % \answerTODO{}
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    % \answerTODO{}
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

